Aspects of Quantum Cosmology

In this thesis, we try to resolve the alleged problem of non-unitarity for various anisotropic cosmological models. Using Wheeler-DeWitt formulation, we quantized the anisotropic models with variable spatial curvature, namely Bianchi II and Bianchi VI. We showed that Hamiltonian of respective models admits self-adjoint extension, thus unitary evolution. We further extended the unitary evolution for higher dimensional anisotropic cosmological models. We also showed that unitarity of the model preserves the Noether symmetry but loses the scale invariance. In later part of this thesis, we showed the equivalence of Jordan and Einstein frames at the quantum level for the flat FRW model. Obtained expressions for wave packet matched exactly in both the frames indicating the equivalence of frames. We also showed that equivalence holds true for various anisotropic quantum cosmological models, i.e., Bianchi I, V, X, LRS Bianchi-I and Kantowski-Sachs models.

==> acknow.tex <==
%\addchaptertocentry{\publication} 
\thispagestyle{plain}
\null\vfil
{\huge\bfseries \centering Acknowledgements \par\vspace{20pt}}
%\addcontentsline{toc}{chapter}{Acknowledgements}
It is only apt that I express my gratitude to all those people who have made the journey to this stage possible. Following only the chronological order, let me start with paying my first respects to my parents. Mere Thank you is not enough for everything you have done for me, for all I am today, and all I have achieved could not have been possible without the urge of learning you planted and nurtured in me. It would take a very long paragraph to thank my family. So, in short, I would like to thank my grandparents, uncles, aunties, brothers, sisters, and everyone else who have their blessing on me. Thank you all for guiding and helping me it every stage of my life in one way or the other.

I can not move ahead without mentioning those invaluable teachers of my earlier years who have played a crucial role in developing and shaping my interest in science. Specially, my high-school teachers, Aditya sir, for fueling my interest in physics and maths. My chemistry teacher Naveen sir had also been an ever encouraging figure to me, and I am forever grateful to you for your encouragement.

I also thank all the teachers of the Physics department of Banaras Hindu University, Varanasi; for not only they kept alive my interest in physics but fueled it with more energy. I thank Dr. Anchal Srivastava, Dr. Bhavani Prasad Mandal, and Dr. Debanand Sa for enabling me to discover my true interests.

The best part of my academic life came when I arrived in IISER-Kolkata. I am most grateful to my research advisor Dr. Nirmalya Ghosh, whose passion for science, curiosity, and positive attitude are extremely contagious. This thesis would not have materialized without your expert guidance, which I know will always be available to me when in need. I thank you for patiently bearing with me for all these years and believing in my capabilities. I am also indebted to you for providing me the plenty of opportunities to explore myself and for teaching me how to be an independent researcher.

I would also like to thank my current collaborators Dr. Ayan Banerjee, Dr. Partha Mitra, Dr.Sourin Das from IISER Kolkata, Dr. Achanta Venugopal from TIFR Mumbai and Dr. Subhasish. Dattagupta from Univ. of Hyderabad for all the encouragement and discussions from which I have learned a lot. I am also grateful to my research progress committee member Dr. Prashanta Panigrahi.

I should also thank all those people who have helped in making my days bearable when I was away from my family. I am thankful to Dr. Sudipta Saha and Dr. Shubham Chandel with whom I was working with on various problems, for the stimulating discussions on various topics and various other personal help and discussions. The list can not be complete without mentioning my other lab members; Dr. Jalpa Soni, Dr. Nandan Kumar Das, Dr. Mandira Pal, Dr. Subir Ray, Rajib Dey, Dr. Chitram Banerjee, Abhishek Kumar, Athira, Niladri, Shyamal, Jeeban, Antariksha, Anwesha, Ajmal, Aneeth, Anchita, Angad, Bhavya, Arindam, Sumit, Sayandip, Jatadhari, Debanuj, and Akshay. Thank you all.

The days at IISER K has been wonderful because of these lovely people being present during my important days at different times. The NSCB 3rd floor group of amazing people like Sachin (Pandu), Sushant (Bandhua), Abhinashji, Deepak, Shashwat, Soumen, Ravi, Akash, Chindu, Pawan, Ashish who are like my family and never made me miss my college or home. And Also, Mayank, Subrata, Rahul, Anand, Raghav, who were always there with interesting discussions and stories, and of course, the Goa trip. The list would be incomplete without mentioning Debashirta, Irina di, Burman da, Chiru da, Shubhro da, Anurag Banerjee, who tolerated me during my stay in IISER Kolkata. At last, I am thankful to all the administrative staff, security personnel, housekeeping staff, and the IISER Kolkata family for providing me the home away from home.

At the end of this fairly long testimonial, I once again thank everyone from whom I have learned something or the other...
\vskip 2cm
\emph{Ankit Kumar Singh}\\
\emph{IISER Kolkata, \today}


==> ch6_paper5.tex <==
\chapter{Title-paper4}


\section{Background}


\subsection{a}





\subsection{b}

\section{Results and discussions}

\section{Conclusion}

==> ch7_paper6.tex <==
\chapter{Title-paper5}


\section{Background}


\subsection{a}





\subsection{b}

\section{Results and discussions}


\section{Conclusion}


==> dedicated.tex <==
    \begin{center}
        \vspace*{1cm}
        

        \vspace{0.5cm}
        \LARGE 
        To \\
        \vspace{1.5cm}
        \LARGE
         My Parents\\
        \vspace{0.5cm} 
         My Uncle \\
        \vspace{0.5cm}
            and \\
        \vspace{0.5cm} 
         My late Grandmother\\

   \end{center}


==> title.tex <==
%\titlehead{\centering {\bf Indian Institution of Science Education and Research (IISER)\\ Kolkata}}

\vspace{-1.50cm}
\titlehead{\centering {\Large Dissertation for obtaining the Doctor of Philosophy (PhD) of Physics}}

\title{\centering The study of swelling kinetics of polyelectrolyte gels}

\author{\Large {\bf Swati Sen}}

%\date{dasas}

\publishers{\includegraphics[width=0.35\textwidth]{iiserklogo.png}}

%\subject{Dissertation for obtaining the Doctor of Philosophy (PhD) of Physics
%}
\date{}

{\Large
\lowertitleback{
\begin{tabular}{L{7cm}L{6cm}}
 Supervisor: & Dr. Arindam Kundagrami \\\\
%Korreferent/in:&\hrulefill\\\\\\
%Tag der mündlichen Prüfung:&\hrulefill\\\\
%Zum Druck genehmigt:&\hrulefill\\\\\\\\
%&\hrulefill\\
%&Dekan
\end{tabular}
}}

\maketitle


==> title3.tex <==
\begin{titlepage}
    \begin{center}
        \vspace*{5cm}
      
      \LARGE   
      \textit{tribute to} \\
        \vspace{1.5cm}
         \LARGE
         \textit{---------TBA-----------} \\
        

   \end{center}
\end{titlepage}


==> title_page.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Vertical Line Title Page 
% LaTeX Template
% Version 1.0 (27/12/12)
%
% This template has been downloaded from:
% http://www.LaTeXTemplates.com
%
% Original author:
% Peter Wilson (herries.press@earthlink.net)
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
% 
% Instructions for using this template:
% This title page compiles as is. If you wish to include this title page in 
% another document, you will need to copy everything before 
% \begin{document} into the preamble of your document. The title page is
% then included using \titleGM within your document.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%----------------------------------------------------------------------------------------
%	PACKAGES AND OTHER DOCUMENT CONFIGURATIONS
%----------------------------------------------------------------------------------------

%\documentclass{book}

\newcommand*{\plogo}{\fbox{$\mathcal{PL}$}} % Generic publisher logo

%----------------------------------------------------------------------------------------
%	TITLE PAGE
%----------------------------------------------------------------------------------------

\newcommand*{\titleGM}{\begingroup % Create the command for including the title page in the document
\hbox{ % Horizontal box
\hspace*{0.005\textwidth} % Whitespace to the left of the title page
\rule{1.5pt}{\textheight} % Vertical line
\hspace*{0.02\textwidth} % Whitespace between the vertical line and title page text
\parbox[b]{0.95\textwidth}{ % Paragraph box which restricts text to less than the width of the page


{\noindent\Huge\bfseries The study of swelling kinetics of polyelectrolyte gels in a salt-free solvent}\\[2\baselineskip] % Title
{\large \textit{Dissertation for obtaining the Doctor of Philosophy (PhD) of Physics}}\\[4\baselineskip] % Tagline or further description
%\vspace{0.2\textheight}
{\Huge \textsc{Swati Sen}} % Author name

\vspace{0.5\textheight} % Whitespace between the title block and the publisher
{\noindent {\Large {\bf Indian Institute of Science Education and Research Kolkata} }}\\[\baselineskip] % Publisher and logo
}}
\endgroup}

%----------------------------------------------------------------------------------------
%	BLANK DOCUMENT
%----------------------------------------------------------------------------------------

%\begin{document}

\pagestyle{empty} % Removes page numbers

\titleGM % This command includes the title page

%\end{document}


==> title_page3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Vertical Line Title Page 
% LaTeX Template
% Version 1.0 (27/12/12)
%
% This template has been downloaded from:
% http://www.LaTeXTemplates.com
%
% Original author:
% Peter Wilson (herries.press@earthlink.net)
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
% 
% Instructions for using this template:
% This title page compiles as is. If you wish to include this title page in 
% another document, you will need to copy everything before 
% \begin{document} into the preamble of your document. The title page is
% then included using \titleGM within your document.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%----------------------------------------------------------------------------------------
%	PACKAGES AND OTHER DOCUMENT CONFIGURATIONS
%----------------------------------------------------------------------------------------

%\documentclass{book}

\newcommand*{\plogo}{\fbox{$\mathcal{PL}$}} % Generic publisher logo

%----------------------------------------------------------------------------------------
%	TITLE PAGE
%----------------------------------------------------------------------------------------

\newcommand*{\titleGM}{\begingroup % Create the command for including the title page in the document
\hbox{ % Horizontal box
\hspace*{0.005\textwidth} % Whitespace to the left of the title page
\rule{1.5pt}{\textheight} % Vertical line
\hspace*{0.02\textwidth} % Whitespace between the vertical line and title page text
\parbox[b]{0.95\textwidth}{ % Paragraph box which restricts text to less than the width of the page

\definecolor{grey}{rgb}{0.9,0.9,0.9}

\colorbox{grey}{
	\parbox[t]{1.0\linewidth}{
		\centering \fontsize{50pt}{25pt}\selectfont
          \vspace*{0.1cm}

{\noindent\Huge\bfseries The study of equilibrium and kinetics of swelling of polymer and polyelectrolyte gels in a salt-free solvent}\\[2\baselineskip] % Title

\vspace*{-0.1cm}
	}
}



{\large \textit{Dissertation for obtaining the Doctor of Philosophy (PhD) of Physics}}\\[4\baselineskip] % Tagline or further description
%\vspace{0.2\textheight}
{\Huge \textsc{Swati Sen}} % Author name

\vspace{0.5\textheight} % Whitespace between the title block and the publisher
{\noindent {\Large {\bf Indian Institute of Science Education and Research Kolkata} }}\\[\baselineskip] % Publisher and logo
}}
\endgroup}

%----------------------------------------------------------------------------------------
%	BLANK DOCUMENT
%----------------------------------------------------------------------------------------

%\begin{document}

\pagestyle{empty} % Removes page numbers

\titleGM % This command includes the title page

%\end{document}

